Linear Progressive Coding for Semantic Communication using Deep Neural Networks

We propose a general method for semantic representation of images and other data using progressive coding. Semantic coding allows for specific pieces of information to be selectively encoded into a set of measurements that can be highly compressed compared to the size of the original raw data. We consider a hierarchical method of coding where a partial amount of semantic information is first encoded a into a coarse representation of the data, which is then refined by additional encodings that add additional semantic information. Such hierarchical coding is especially well-suited for semantic communication i.e. transferring semantic information over noisy channels. Our proposed method can be considered as a generalization of both progressive image compression and source coding for semantic communication. We present results from experiments on the MNIST and CIFAR-10 datasets that show that progressive semantic coding can provide timely previews of semantic information with a small number of initial measurements while achieving overall accuracy and efficiency comparable to non-progressive methods.

==> expdetails.tex <==

In the first part of this effort, the MNIST dataset is invoked here for a two-task execution, with the goal of achieving a macro-level coarse refinement in Task 1, and achieve a lower level, or finer, solution as the objective of Task 2. Here, in the context of implementing the MNIST dataset, the Task 1 objective is to convey even or oddness of an input MNIST image output. In Task 2, the objective is to deliver number recognition for the same respective input image to the overall framework. In Task 1, the compressed output from Sample 1 is characterized with a dimension of [1 a], where the coefficients of the compressing fully connected layer in Sample 1 are learned from training the overall neural network for achieving the objective of Task 1. The Sample 2 output has an additional output contribution of dimension [1 b] to the overall compressed dimension, [1 (a+b)]. The [1 a] dimension relates to fixed component of Sample 2. The weights and biases of the trained neural network from Sample 1, are then transferred to a compressive custom connected layer in Sample 2, where the weights and biases contribution from Task 1 is held fixed, and only the weights and biases from the introduced dimension of b are trained and learnable.

In the process of developing this progressive image coding framework, it is imperative to develop a bounding structure to ensure proper performance of the individual semantic tasks. The next order of business is to provide a basis of bounding constraints for our problem setup. The bounding constraints to be portrayed are demonstrated in Figure [x]. In this Figure, the initial coarse experiment is executed in Column 5, and the follow-up Fine experiment result is detailed in Column 6. All of the remainder columns are related to the expected, relative minima and maxima performances, or anticipated bounding cases, and have an input argument associated with the respective combination: (a,b). The value of ‘a’ pertains to the compressed coarse output dimension, and the value of b relates to the compressed fine output dimension. Columns 1 – 4 are the identical functional experiments as those listed in Columns 7 – 10, however with different input arguments related to the (a,b) pair. The different input arguments demonstrate the bounding conditions that are executed to compare against the Coarse and Fine experiment results, and to infer the practicality of achieved results.

In Column 1, the objective of this experiment is to determine the probability of the classification outcome to complete the coarse task, in order to classify the higher order label. In the case of the MNIST dataset, the coarse goal is to identify if the number is even or odd. 

In Column 2, the objective of this experiment is to execute the classification of the fine, or in other words, the lower order classification. In the context of the MNIST dataset, this would result in performing number recognition on the respective, input image. In this case, there are no additional weights or biases solved for during training in the compression layer, and this condition is indicated by the b=0 input argument. In execution of the experiment, the weights and biases of the compression layer from Column 1 are utilized here in the Column 2 compression layer. No other weights and biases are trained in the Compression layer, for this experiment.

In Column 3, the execution of this experiment has a dependency from the execution of the Column 4 experiment. The Column 3 experiment applies the weights and biases from the compression layer from the Column 4 experiment, and trains the neural network to achieve the coarse classification.

In Column 4, the goal of this respective experiment is to perform fine classification, first, with the secondary goal, of re-purposing the final, trained weights and biases from the compression layer in the Column 3 semantic task.  

The experiments related to Columns 7 – 10, are identical in function, comparatively and respectively to Columns 1 – 4. 

The bounding criterion effectively implemented in this effort entails that the lower bound for statistical performance is established by the experiments in Columns 1 – 4, since only the singular value of a, is the argument for all of the respective input parameters, translating to smaller allowed compressed measurements. For the cases explained in Columns 7 – 10, the non-zero input parameter changes from the value of ‘a’ to ‘a+b’, where a and b are non-negative integer values. Hence, the compressed measurement increases, in size, and would reasonably reflect a higher probability performance for classification. With respect to the combined coarse and fine semantic tasks, the coarse task of Column 6 is effectively equal to the conducted experiment of Column 1. There is no direct equivalent experiment in the entire set of experiments for the fine task of Column 6. The compressed measurement size of the fine task is [1  (a+b)]. The compressed measurement size of fine task in Column 10 is also [1 (a+b)], however these two experiments are not equivalent. The fine experiment of Column 6 involves having a fixed component of weights and biases in the compression layer imported from Column 5’s coarse task, therefore there is a fixed and a learnable component in the compression layer for the neural network of Column 6. In Column 10, the compression layer is derived entirely of learnable components, and no fixed components. In this scenario, the task of Column 10 essentially creates the upper bound to the performance for the composite fixed-learnable, fine task of Column 6. 

In Column 11, the goal of this specific experiment pertains to a verification-associated task. The compressed calculated outputs of dimension [1 b], or activations at the compressed data point, from the execution of the fine task, are used as the input, at the compress point as input data in the coarse task. This experiment effectively serves as a conditional confirmation step, to verify that if provided the the compressed layer outputs from the fine task, to determine the likelihood that the coarse task was executed accurately. This experiments provides a measure of added confidence in the overall 2-stage Coarse-Fine Semantic task execution. 

